Impossibility results for fair representations

With the growing awareness to fairness in machine learning and the realization of the central role that data representation has in data processing tasks, there is an obvious interest in notions of fair data representations. The goal of such representations is that a model trained on data under the representation (e.g., a classifier) will be guaranteed to respect some fairness constraints. Such representations are useful when they can be fixed for training models on various different tasks and also when they serve as data filtering between the raw data (known to the representation designer) and potentially malicious agents that use the data under the representation to learn predictive models and make decisions. A long list of recent research papers strive to provide tools for achieving these goals. However, we prove that this is basically a futile effort. Roughly stated, we prove that no representation can guarantee the fairness of classifiers for different tasks trained using it; even the basic goal of achieving label-independent Demographic Parity fairness fails once the marginal data distribution shifts. More refined notions of fairness, like Odds Equality, cannot be guaranteed by a representation that does not take into account the task specific labeling rule with respect to which such fairness will be evaluated (even if the marginal data distribution is known a priory). Furthermore, except for trivial cases, no representation can guarantee Odds Equality fairness for any two different tasks, while allowing accurate label predictions for both. While some of our conclusions are intuitive, we formulate (and prove) crisp statements of such impossibilities, often contrasting impressions conveyed by many recent works on fair representations.

==> references.bib.tex <==
@inproceedings{kour2014real,
  title={Real-time segmentation of on-line handwritten arabic script},
  author={Kour, George and Saabne, Raid},
  booktitle={Frontiers in Handwriting Recognition (ICFHR), 2014 14th International Conference on},
  pages={417--422},
  year={2014},
  organization={IEEE}
}

@inproceedings{kour2014fast,
  title={Fast classification of handwritten on-line Arabic characters},
  author={Kour, George and Saabne, Raid},
  booktitle={Soft Computing and Pattern Recognition (SoCPaR), 2014 6th International Conference of},
  pages={312--318},
  year={2014},
  organization={IEEE}
}

@article{hadash2018estimate,
  title={Estimate and Replace: A Novel Approach to Integrating Deep Neural Networks with Existing Applications},
  author={Hadash, Guy and Kermany, Einat and Carmeli, Boaz and Lavi, Ofer and Kour, George and Jacovi, Alon},
  journal={arXiv preprint arXiv:1804.09028},
  year={2018}
}

}
%%% ====================================================================
%%%  BibTeX-file{
%%%     author          = "Gerry Murray",
%%%     version         = "1.2",
%%%     date            = "2 April 2012",
%%%     filename        = "acmsmall-sample-bibfile.bib",
%%%     address         = "ACM, NY",
%%%     email           = "murray at hq.acm.org",
%%%     codetable       = "ISO/ASCII",
%%%     keywords        = "ACM Reference Format, bibliography, citation, references",
%%%     supported       = "yes",
%%%     docstring       = "This BibTeX database file contains 'bibdata' entries
%%%                        that 'match' the examples provided in the Specifications Document
%%%                        AND, also, 'legacy'-type bibs. It should assist authors in
%%%                        choosing the 'correct' at-bibtype and necessary bib-fields
%%%                        so as to obtain the appropriate ACM Reference Format output.
%%%                        It also contains many 'Standard Abbreviations'. "
%%%  }
%%% ====================================================================

% Journals

% First the Full Name is given, then the abbreviation used in the AMS Math
% Reviews, with an indication if it could not be found there.
% Note the 2nd overwrites the 1st, so swap them if you want the full name.

 %{AMS}
 @String{AMSTrans = "American Mathematical Society Translations" }
 @String{AMSTrans = "Amer. Math. Soc. Transl." }
 @String{BullAMS = "Bulletin of the American Mathematical Society" }
 @String{BullAMS = "Bull. Amer. Math. Soc." }
 @String{ProcAMS = "Proceedings of the American Mathematical Society" }
 @String{ProcAMS = "Proc. Amer. Math. Soc." }
 @String{TransAMS = "Transactions of the American Mathematical Society" }
 @String{TransAMS = "Trans. Amer. Math. Soc." }

 %ACM
 @String{CACM = "Communications of the {ACM}" }
 @String{CACM = "Commun. {ACM}" }
 @String{CompServ = "Comput. Surveys" }
 @String{JACM = "J. ACM" }
 @String{ACMMathSoft = "{ACM} Transactions on Mathematical Software" }
 @String{ACMMathSoft = "{ACM} Trans. Math. Software" }
 @String{SIGNUM = "{ACM} {SIGNUM} Newsletter" }
 @String{SIGNUM = "{ACM} {SIGNUM} Newslett." }

 @String{AmerSocio = "American Journal of Sociology" }
 @String{AmerStatAssoc = "Journal of the American Statistical Association" }
 @String{AmerStatAssoc = "J. Amer. Statist. Assoc." }
 @String{ApplMathComp = "Applied Mathematics and Computation" }
 @String{ApplMathComp = "Appl. Math. Comput." }
 @String{AmerMathMonthly = "American Mathematical Monthly" }
 @String{AmerMathMonthly = "Amer. Math. Monthly" }
 @String{BIT = "{BIT}" }
 @String{BritStatPsych = "British Journal of Mathematical and Statistical
          Psychology" }
 @String{BritStatPsych = "Brit. J. Math. Statist. Psych." }
 @String{CanMathBull = "Canadian Mathematical Bulletin" }
 @String{CanMathBull = "Canad. Math. Bull." }
 @String{CompApplMath = "Journal of Computational and Applied Mathematics" }
 @String{CompApplMath = "J. Comput. Appl. Math." }
 @String{CompPhys = "Journal of Computational Physics" }
 @String{CompPhys = "J. Comput. Phys." }
 @String{CompStruct = "Computers and Structures" }
 @String{CompStruct = "Comput. \& Structures" }
 @String{CompJour = "The Computer Journal" }
 @String{CompJour = "Comput. J." }
 @String{CompSysSci = "Journal of Computer and System Sciences" }
 @String{CompSysSci = "J. Comput. System Sci." }
 @String{Computing = "Computing" }
 @String{ContempMath = "Contemporary Mathematics" }
 @String{ContempMath = "Contemp. Math." }
 @String{Crelle = "Crelle's Journal" }
 @String{GiornaleMath = "Giornale di Mathematiche" }
 @String{GiornaleMath = "Giorn. Mat." } % didn't find in AMS MR., ibid.

 %IEEE
 @String{Computer = "{IEEE} Computer" }
 @String{IEEETransComp = "{IEEE} Transactions on Computers" }
 @String{IEEETransComp = "{IEEE} Trans. Comput." }
 @String{IEEETransAC = "{IEEE} Transactions on Automatic Control" }
 @String{IEEETransAC = "{IEEE} Trans. Automat. Control" }
 @String{IEEESpec = "{IEEE} Spectrum" } % didn't find in AMS MR
 @String{ProcIEEE = "Proceedings of the {IEEE}" }
 @String{ProcIEEE = "Proc. {IEEE}" } % didn't find in AMS MR
 @String{IEEETransAeroElec = "{IEEE} Transactions on Aerospace and Electronic
     Systems" }
 @String{IEEETransAeroElec = "{IEEE} Trans. Aerospace Electron. Systems" }

 @String{IMANumerAna = "{IMA} Journal of Numerical Analysis" }
 @String{IMANumerAna = "{IMA} J. Numer. Anal." }
 @String{InfProcLet = "Information Processing Letters" }
 @String{InfProcLet = "Inform. Process. Lett." }
 @String{InstMathApp = "Journal of the Institute of Mathematics and
     its Applications" }
 @String{InstMathApp = "J. Inst. Math. Appl." }
 @String{IntControl = "International Journal of Control" }
 @String{IntControl = "Internat. J. Control" }
 @String{IntNumerEng = "International Journal for Numerical Methods in
     Engineering" }
 @String{IntNumerEng = "Internat. J. Numer. Methods Engrg." }
 @String{IntSuper = "International Journal of Supercomputing Applications" }
 @String{IntSuper = "Internat. J. Supercomputing Applic." } % didn't find
%% in AMS MR
 @String{Kibernetika = "Kibernetika" }
 @String{JResNatBurStand = "Journal of Research of the National Bureau
     of Standards" }
 @String{JResNatBurStand = "J. Res. Nat. Bur. Standards" }
 @String{LinAlgApp = "Linear Algebra and its Applications" }
 @String{LinAlgApp = "Linear Algebra Appl." }
 @String{MathAnaAppl = "Journal of Mathematical Analysis and Applications" }
 @String{MathAnaAppl = "J. Math. Anal. Appl." }
 @String{MathAnnalen = "Mathematische Annalen" }
 @String{MathAnnalen = "Math. Ann." }
 @String{MathPhys = "Journal of Mathematical Physics" }
 @String{MathPhys = "J. Math. Phys." }
 @String{MathComp = "Mathematics of Computation" }
 @String{MathComp = "Math. Comp." }
 @String{MathScand = "Mathematica Scandinavica" }
 @String{MathScand = "Math. Scand." }
 @String{TablesAidsComp = "Mathematical Tables and Other Aids to Computation" }
 @String{TablesAidsComp = "Math. Tables Aids Comput." }
 @String{NumerMath = "Numerische Mathematik" }
 @String{NumerMath = "Numer. Math." }
 @String{PacificMath = "Pacific Journal of Mathematics" }
 @String{PacificMath = "Pacific J. Math." }
 @String{ParDistComp = "Journal of Parallel and Distributed Computing" }
 @String{ParDistComp = "J. Parallel and Distrib. Comput." } % didn't find
%% in AMS MR
 @String{ParComputing = "Parallel Computing" }
 @String{ParComputing = "Parallel Comput." }
 @String{PhilMag = "Philosophical Magazine" }
 @String{PhilMag = "Philos. Mag." }
 @String{ProcNAS = "Proceedings of the National Academy of Sciences
                    of the USA" }
 @String{ProcNAS = "Proc. Nat. Acad. Sci. U. S. A." }
 @String{Psychometrika = "Psychometrika" }
 @String{QuartMath = "Quarterly Journal of Mathematics, Oxford, Series (2)" }
 @String{QuartMath = "Quart. J. Math. Oxford Ser. (2)" }
 @String{QuartApplMath = "Quarterly of Applied Mathematics" }
 @String{QuartApplMath = "Quart. Appl. Math." }
 @String{RevueInstStat = "Review of the International Statisical Institute" }
 @String{RevueInstStat = "Rev. Inst. Internat. Statist." }

 %SIAM
 @String{JSIAM = "Journal of the Society for Industrial and Applied
     Mathematics" }
 @String{JSIAM = "J. Soc. Indust. Appl. Math." }
 @String{JSIAMB = "Journal of the Society for Industrial and Applied
     Mathematics, Series B, Numerical Analysis" }
 @String{JSIAMB = "J. Soc. Indust. Appl. Math. Ser. B Numer. Anal." }
 @String{SIAMAlgMeth = "{SIAM} Journal on Algebraic and Discrete Methods" }
 @String{SIAMAlgMeth = "{SIAM} J. Algebraic Discrete Methods" }
 @String{SIAMAppMath = "{SIAM} Journal on Applied Mathematics" }
 @String{SIAMAppMath = "{SIAM} J. Appl. Math." }
 @String{SIAMComp = "{SIAM} Journal on Computing" }
 @String{SIAMComp = "{SIAM} J. Comput." }
 @String{SIAMMatrix = "{SIAM} Journal on Matrix Analysis and Applications" }
 @String{SIAMMatrix = "{SIAM} J. Matrix Anal. Appl." }
 @String{SIAMNumAnal = "{SIAM} Journal on Numerical Analysis" }
 @String{SIAMNumAnal = "{SIAM} J. Numer. Anal." }
 @String{SIAMReview = "{SIAM} Review" }
 @String{SIAMReview = "{SIAM} Rev." }
 @String{SIAMSciStat = "{SIAM} Journal on Scientific and Statistical
     Computing" }
 @String{SIAMSciStat = "{SIAM} J. Sci. Statist. Comput." }

 @String{SoftPracExp = "Software Practice and Experience" }
 @String{SoftPracExp = "Software Prac. Experience" } % didn't find in AMS MR
 @String{StatScience = "Statistical Science" }
 @String{StatScience = "Statist. Sci." }
 @String{Techno = "Technometrics" }
 @String{USSRCompMathPhys = "{USSR} Computational Mathematics and Mathematical
     Physics" }
 @String{USSRCompMathPhys = "{U. S. S. R.} Comput. Math. and Math. Phys." }
 @String{VLSICompSys = "Journal of {VLSI} and Computer Systems" }
 @String{VLSICompSys = "J. {VLSI} Comput. Syst." }
 @String{ZAngewMathMech = "Zeitschrift fur Angewandte Mathematik und
     Mechanik" }
 @String{ZAngewMathMech = "Z. Angew. Math. Mech." }
 @String{ZAngewMathPhys = "Zeitschrift fur Angewandte Mathematik und Physik" }
 @String{ZAngewMathPhys = "Z. Angew. Math. Phys." }

% Publishers % ================================================= |

 @String{Academic = "Academic Press" }
 @String{ACMPress = "{ACM} Press" }
 @String{AdamHilger = "Adam Hilger" }
 @String{AddisonWesley = "Addison-Wesley" }
 @String{AllynBacon = "Allyn and Bacon" }
 @String{AMS = "American Mathematical Society" }
 @String{Birkhauser = "Birkha{\"u}ser" }
 @String{CambridgePress = "Cambridge University Press" }
 @String{Chelsea = "Chelsea" }
 @String{ClaredonPress = "Claredon Press" }
 @String{DoverPub = "Dover Publications" }
 @String{Eyolles = "Eyolles" }
 @String{HoltRinehartWinston = "Holt, Rinehart and Winston" }
 @String{Interscience = "Interscience" }
 @String{JohnsHopkinsPress = "The Johns Hopkins University Press" }
 @String{JohnWileySons = "John Wiley and Sons" }
 @String{Macmillan = "Macmillan" }
 @String{MathWorks = "The Math Works Inc." }
 @String{McGrawHill = "McGraw-Hill" }
 @String{NatBurStd = "National Bureau of Standards" }
 @String{NorthHolland = "North-Holland" }
 @String{OxfordPress = "Oxford University Press" }  %address Oxford or London?
 @String{PergamonPress = "Pergamon Press" }
 @String{PlenumPress = "Plenum Press" }
 @String{PrenticeHall = "Prentice-Hall" }
 @String{SIAMPub = "{SIAM} Publications" }
 @String{Springer = "Springer-Verlag" }
 @String{TexasPress = "University of Texas Press" }
 @String{VanNostrand = "Van Nostrand" }
 @String{WHFreeman = "W. H. Freeman and Co." }

%Entries

@inproceedings{hardt2016equality,
    title     = {Equality of opportunity in supervised learning},
	author    = {Hardt, Moritz and Price, Eric and Srebro, Nathan},
	booktitle = {NIPS},
	year      = {2016}
}

@inproceedings{grgic2018beyond,
	title     = {Beyond Distributive Fairness in Algorithmic Decision Making: Feature Selection for Procedurally Fair Learning},
	author    = {Grgic-Hlaca, Nina and Bilal Zafar, Muhammad and P. Gummadi, Krishna and Weller, Adrian},
	booktitle = {AAAI},
	year      = {2018}
}

@inproceedings{kamishima2011fairness,
	title     = {Fairness-aware learning through regularization approach},
	author    = {Kamishima, Toshihiro and Akaho, Shotaro and Sakuma, Jun},
	booktitle = {IEEE 11th International Conference on Data Mining Workshops},
	year      = {2011}
}

@inproceedings{chen2018my,
	title     = {Why is my classifier discriminatory?},
	author    = {Chen, Irene and Johansson, Fredrik D and Sontag, David},
	booktitle = {NIPS},
	year      = {2018}
}

@inproceedings{zemel2013learning,
	title     = {Learning fair representations},
	author    = {Zemel, Rich and Wu, Yu and Swersky, Kevin and Pitassi, Toni and Dwork, Cynthia},
	booktitle = {ICML},
	year      = {2013}
}

@inproceedings{Dwork2012,
	author    = {Dwork, Cynthia and Hardt, Moritz and Pitassi, Toniann and Reingold, Omer and S. Zemel, Richard},
	editor    = {Shafi Goldwasser},
	title     = {Fairness through awareness},
	booktitle = {Innovations in Theoretical Computer Science},
	year      = {2012}
}

@inproceedings{DBLP:conf/icml/zemmel2019,
	author    = {Creager, Elliot and Madras, David and Jacobsen, Joern-Henrik and Weis, Marissa and Swersky, Kevin and Pitassi, Toniann and Zemel, Richard},
	title     = {Flexibly Fair Representation Learning by Disentanglement},
	booktitle = {ICML},
	year      = {2019}
}


@inproceedings{joseph2018meritocratic,
	title     = {Meritocratic fairness for infinite and contextual bandits},
	author    = {Joseph, Matthew and Kearns, Michael and Morgenstern, Jamie and Neel, Seth and Roth, Aaron},
	booktitle = {Proceedings of the 2018 AAAI/ACM Conference on AI, Ethics, and Society},
	year      = {2018}
}

@inproceedings{joseph2016fairness,
	title     = {Fairness in learning: Classic and contextual bandits},
	author    = {Joseph, Matthew and Kearns, Michael and Morgenstern, Jamie H and Roth, Aaron},
	booktitle = {NIPS},
	year      = {2016}
}

@inproceedings{kim2018fairness,
	title     = {Fairness through computationally-bounded awareness},
	author    = {Kim, Michael and Reingold, Omer and Rothblum, Guy},
	booktitle = {NIPS},
	year      = {2018}
}

@inproceedings{pmlr-v80-madras18a,
	title     = {Learning Adversarially Fair and Transferable Representations},
	author    = {Madras, David and Creager, Elliot and Pitassi, Toniann and Zemel, Richard},
	booktitle = {ICML},
	year      = {2018}
}


@inproceedings{DBLP:journals/corr/EdwardsS15,
    author    = {Harrison Edwards and Amos J. Storkey},
	title     = {Censoring Representations with an Adversary},
	booktitle = {ICLR},
	year      = {2016}
}

@inproceedings{kleinberg2019simplicity,
	author    = {Kleinberg, Jon and Mullainathan, Sendhil},
	title     = {Simplicity Creates Inequity: Implications for Fairness, Stereotypes, and Interpretability},
	booktitle = {EC},
	year      = {2019}
}

@inproceedings{Zhang_2018,
	title     = {Mitigating Unwanted Biases with Adversarial Learning},
	booktitle = {AAAI/ACM Conference on AI, Ethics, and Society},
	author    = {Zhang, Brian Hu and Lemoine, Blake and Mitchell, Margaret},
	year      = {2018},
}

@article{shai2010domain,
	author  = {Ben-David, Shai and Blitzer, John and Crammer, Koby and Kulesza, Alex and Pereira, Fernando and Vaughan, Jennifer Wortman},
	title   = {A Theory of Learning from Different Domains},
	journal = {Mach. Learn.},
	volume  = {79},
	number  = {1–2},
	year    = {2010}
}

@article{garg2019tracking,
	author  = {Garg, Sumegha and Kim, Michael P and Reingold, Omer},
	title   = {Tracking and Improving Information in the Service of Fairness},
	journal = {CoRR},
	volume  = {abs/1904.09942},
	year    = {2019}
}

@article{corbett2018measure,
	title   = {The measure and mismeasure of fairness: A critical review of fair machine learning},
	author  = {Corbett-Davies, Sam and Goel, Sharad},
	journal = {CoRR},
	volume  = {abs/1808.00023},
	year    = {2019}
}

@article{zhao2019conditional,
	title   = {Conditional Learning of Fair Representations},
	author  = {Han Zhao and Amanda Coston and Tameem Adel and Geoffrey J. Gordon},
	journal = {CoRR},
	volume  = {abs/1910.07162},
	year    = {2019}
}

@article{jiang2019wasserstein,
	title   = {Wasserstein Fair Classification},
	author  = {Ray Jiang and Aldo Pacchiano and Tom Stepleton and Heinrich Jiang and Silvia Chiappa},
	journal = {CoRR},
	volume  = {abs/1907.12059},
	year    = {2019}
}

@article{zhao2019inherent,
	title   = {Inherent Tradeoffs in Learning Fair Representations},
	author  = {Han Zhao and Geoffrey J. Gordon},
	journal = {CoRR},
	volume  = {abs/1906.08386},
	year    = {2019}
}

@article{DBLP:journals/corr/BeutelCZC17,
	author    = {Alex Beutel and Jilin Chen and	Zhe Zhao and Ed H. Chi},
	title     = {Data Decisions and Theoretical Implications when Adversarially Learning
	Fair Representations},
	journal   = {CoRR},
	volume    = {abs/1707.00075},
	year      = {2017}
}

@article{kallus2018residual,
	title   = {Residual unfairness in fair machine learning from prejudiced data},
	author  = {Kallus, Nathan and Zhou, Angela},
	journal = {CoRR},
	volume  = {abs/1806.02887},
	year    = {2018}
}

@article{hashimoto2018fairness,
	title   = {Fairness without demographics in repeated loss minimization},
	author  = {Hashimoto, Tatsunori B and Srivastava, Megha and Namkoong, Hongseok and Liang, Percy},
	journal = {CoRR},
	volume  = {abs/1806.08010},
	year    = {2018}
}

@article{ilvento2019metric,
	title   = {Metric learning for individual fairness},
	author  = {Ilvento, Christina},
	journal = {CoRR},
	volume  = {abs/1906.00250},
	year    = {2019}
}

@article{rothblum2018probably,
	title   = {Probably approximately metric-fair learning},
	author  = {Rothblum, Guy N and Yona, Gal},
	journal = {CoRR},
	volume  = {abs/1803.03242},
	year    = {2018}
}

@article{lees2019fairness,
	title   = {Fairness Sample Complexity and the Case for Human Intervention},
	author  = {Lees, Alyssa Whitlock and Balashankar, Ananth},
	journal = {CoRR},
	volume  = {abs/1910.11452},
	year    = {2019}
}

@article{barocas2017fairness,
	title   = {Fairness in machine learning},
	author  = {Barocas, Solon and Hardt, Moritz and Narayanan, Arvind},
	journal = {NIPS Tutorial},
	year    = {2017}
}

@article{berk2018fairness,
	title   = {Fairness in criminal justice risk assessments: The state of the art},
	author  = {Berk, Richard and Heidari, Hoda and Jabbari, Shahin and Kearns, Michael and Roth, Aaron},
	journal = {Sociological Methods \& Research},
	year    = {2018}
}

@techreport{doleac2016does,
	title       = {Does “ban the box” help or hurt low-skilled workers? Statistical discrimination and employment outcomes when criminal histories are hidden},
	author      = {Doleac, Jennifer L and Hansen, Benjamin},
	year        = {2016},
	institution = {National Bureau of Economic Research}
}

@techreport{Samarati98protectingprivacy,
	author = {Pierangela Samarati and Latanya Sweeney},
	title = {Protecting Privacy when Disclosing Information: k-Anonymity and Its Enforcement through Generalization and Suppression},
	year = {1998}
}


@article{Sweeney02kanonymity,
  author    = {Latanya Sweeney},
  title     = {k-Anonymity: {A} Model for Protecting Privacy},
  journal   = {Int. J. Uncertain. Fuzziness Knowl. Based Syst.},
  volume    = {10},
  number    = {5},
  pages     = {557--570},
  year      = {2002}
}



@inproceedings{adel2019one,
  title={One-network adversarial fairness},
  author={Adel, Tameem and Valera, Isabel and Ghahramani, Zoubin and Weller, Adrian},
  booktitle={AAAI},
  year={2019}
}

@article{agan2018ban,
  title={Ban the box, criminal records, and racial discrimination: A field experiment},
  author={Agan, Amanda and Starr, Sonja},
  journal={The Quarterly Journal of Economics},
  volume={133},
  number={1},
  pages={191--235},
  year={2018},
  publisher={Oxford University Press}
}

@inproceedings{mcnamara2019costs,
  title={Costs and benefits of fair representation learning},
  author={McNamara, Daniel and Ong, Cheng Soon and Williamson, Robert C},
  booktitle={Proceedings of the 2019 AAAI/ACM Conference on AI, Ethics, and Society},
  pages={263--270},
  year={2019}
}

@article{oneto2019learning,
  title={Learning fair and transferable representations},
  author={Oneto, Luca and Donini, Michele and Maurer, Andreas and Pontil, Massimiliano},
  journal={arXiv preprint arXiv:1906.10673},
  year={2019}
}

@inproceedings{chen2018my,
  title={Why is my classifier discriminatory?},
  author={Chen, Irene and Johansson, Fredrik D and Sontag, David},
  booktitle={Advances in Neural Information Processing Systems},
  pages={3539--3550},
  year={2018}
}

@article{balashankar2019fairness,
  title={Fairness Sample Complexity and the Case for Human Intervention},
  author={Balashankar, Ananth and Lees, Alyssa},
  journal={arXiv preprint arXiv:1910.11452},
  year={2019}
}

@article{zelaya2019parametrised,
  title={Parametrised data sampling for fairness optimisation},
  author={Zelaya, V and Missier, Paolo and Prangle, Dennis},
  journal={KDD XAI},
  year={2019}
}

@inproceedings{song2019learning,
  title={Learning controllable fair representations},
  author={Song, Jiaming and Kalluri, Pratyusha and Grover, Aditya and Zhao, Shengjia and Ermon, Stefano},
  booktitle={The 22nd International Conference on Artificial Intelligence and Statistics},
  pages={2164--2173},
  year={2019}
}

@article{KleinbergMR16,
  author    = {Jon M. Kleinberg and
               Sendhil Mullainathan and
               Manish Raghavan},
  title     = {Inherent Trade-Offs in the Fair Determination of Risk Scores},
  journal   = {CoRR},
  volume    = {abs/1609.05807},
  year      = {2016}

}

@inproceedings{CalmonWVRV17,
  author    = {Fl{\'{a}}vio du Pin Calmon and
               Dennis Wei and
               Bhanukiran Vinzamuri and
               Karthikeyan Natesan Ramamurthy and
               Kush R. Varshney},
  title     = {Optimized Pre-Processing for Discrimination Prevention},
  booktitle = {Advances in Neural Information Processing Systems 30},
  pages     = {3992--4001},
  year      = {2017},
  }


@inproceedings{KleinbergMR17,
  author    = {Jon M. Kleinberg and
               Sendhil Mullainathan and
               Manish Raghavan},
  editor    = {Christos H. Papadimitriou},
  title     = {Inherent Trade-Offs in the Fair Determination of Risk Scores},
  booktitle = {8th Innovations in Theoretical Computer Science Conference, {ITCS}
               2017, January 9-11, 2017, Berkeley, CA, {USA}},
}
